To Explain or Not to Explain: A Study on the Necessity of Explanations for Autonomous Vehicles

Explainable AI, in the context of autonomous systems, like self-driving cars, has drawn broad interests from researchers. Recent studies have found that providing explanations for autonomous vehicles' actions has many benefits (e.g., increased trust and acceptance), but put little emphasis on when an explanation is needed and how the content of explanation changes with driving context. In this work, we investigate which scenarios people need explanations and how the critical degree of explanation shifts with situations and driver types. Through a user experiment, we ask participants to evaluate how necessary an explanation is and measure the impact on their trust in self-driving cars in different contexts. Moreover, we present a self-driving explanation dataset with first-person explanations and associated measures of the necessity for 1103 video clips, augmenting the Berkeley Deep Drive Attention dataset. Our research reveals that driver types and driving scenarios dictate whether an explanation is necessary. In particular, people tend to agree on the necessity for near-crash events but hold different opinions on ordinary or anomalous driving situations.

==> 05-model.tex <==
\section{Model}
\subsection{Overview}
\begin{figure*}[h!]
  \centering
  \includegraphics[width=2.00\columnwidth]{figures/model_architecture.png}
  \caption{Model Architecture. The goal of our model is to identify explanation moments in real-time. The input is a sliding window of video frames, which lasts for four seconds, and it outputs a binary decision on whether to generate an explanation at the end of the input video. First, the model generates a temporal representation from the video data. In particular, we use the foveal feature map, which the model focuses on extracting visual features at the human gaze regions for each frame, proposed by Xia Y., et al. Then, we use a set of fully connected layers to classify the visual features so that we can output a necessity logit at the end.} \label{fig:model-architecture}
\end{figure*}
Our user study suggests that the explanation necessity has to be analyzed on a case-by-case basis. To predict the need for explanation of a particular scenario, we propose a classification model that can predict in real-time about whether a person needs an explanation. The proposed solution can be combined with the state-of-the-art explanation model to generate a text-based explanation at the right moment. The model is trained on our explanation dataset. The input of the model is image data at each time frame. The model outputs a time series of binary decisions for explanation. The architecture of the model is in Figure \ref{fig:model-architecture}.

For this task, we considered it as a classification problem instead of a regression problem. The reason is that, due to the labeling noise by a human, the annotated necessity score can only reflect a relative level of explanation necessity instead of the absolute value. Therefore, we transformed the regression task to a classification task by introducing a pre-specified necessity threshold, $p_0$. The threshold, $p_0$ is influenced by human personal related properties, like driver types. For this paper, we assume $p_0$ is available directly. We leave how we should infer about the threshold value $p_0$ based on different personal attributes for future work.

\subsection{Task \& Notation}
The data of the model is a sliding window of video which lasts for four seconds, and a binary label $y$ indicating explanation necessity at the end of the video.  Our task is to train a classifier $f$ to predict whether an explanation is necessary at the end of the input video clip:
\begin{equation}
    \hat{y}_{i=N} = sgn(f(V) - \sigma),
\end{equation}
where $\hat{y}$ represents the predicted explanation necessity, $i$ represents the frame index (1,2,..,N), $V$ is the input video frame sequence, $\sigma$ is explanation necessity threshold that depends on the passengers' attributes (e.g., driver types), and  $sgn$ represents sign function.

\subsection{Model Detail}
First, the model generates a temporal representation of the image for the last frame in the video. To generate visual features from video frames, we use the Foveal Visual Encoder~\cite{foveal}, proposed by Xia Y. et al., \footnote{Compared with Imagenet pre-trained Alexnet features, the foveal features improved our test AUC from 9.9\% to 24.6\%}. The proposed image encoder predicts small regions where human eyes will focus on each frame, then extracts the image features only for the focused area from a high-resolution video. Then, our model passes those frame features ($A_i$ in Figure \ref{fig:model-architecture}) into Conv2dGRU module~\cite{NIPS2015_5955} and several convolution layers to generate a temporal-spatial representation, $v_i^s$ for each frame $i$, where i = 1,2,..., N and $s$ stands for \textit{spatial}. We extract the output of the last frame, $v^s_{i=N}$, for the next step, where $v^s_{i=N} \in \mathbb{R}^3$.

The model converts the previous spatial features, $v^s_{i=N}$, into a linear representation, $v_{i=N} \in \mathbb{R}$, in the spatial transform module. With the benefits of zero information loss, the model flattens the spatial features directly. We also experimented with the weighted sum approach across spatial locations, suggested by Kim J., et al. in Equation (1) of their paper~\cite{BDDX} for their context vector construction. However, the performance decreased due to information loss during their feature compression across spatial locations.

We concatenate the visual features, $v_{i=N}$ and acceleration, $a_{i=N}$ together. Then, we use several fully connected layers with ReLU nonlinear, BatchNorm~\cite{10.5555/3045118.3045167}, and dropout layers followed. The last step is to use Sigmoid function to generate predicted necessity scores, $\hat{y}$, where $\hat{y} \in [0,1]$. We use Binary Cross-Entropy Loss as our loss function.

In summary, we build a recurrent model to learn explanation necessity. Through our comparison study on different model architecture, we found the foveal feature encoder has better performance in terms of test AUC over Alexnet pre-trained network, even though the foveal feature encoder has information loss on unattended regions at each frame. On the other hand, we learned that flattening works better than the weighted sum proposed by \cite{BDDX} in the Spatial Transform Module for our purpose.

\subsection{Training Details}
We split our dataset into a 70\% training set, a 10\% validation set,  and a 20\% test set. We sampled the video frames at 10 Hz. Then, we extracted training data for video with a sliding window size of 40 frames, (i.e., 4 seconds). For those data piece that has explanation necessity score higher than the specific necessity threshold, we extracted the video window with its end index within the critical time interval (described in the Dataset section) and marked the explanation label as 1. For the rest, we randomly sliced a window with a size of 40 frames in the videos and marked as 0.

We use Adam optimizer with a learning rate of 1e-2, alpha 0.999. The dropout rate is 0.7. To reduce the data imbalance, we did a weighted sampling based on the explanation necessity labels. We set the batch size to be the same as the size of our training dataset to help converge faster. The training of our model took around 1 hour on Nvidia Tesla V100 GPU with 16GB GPU memory, for 300 epochs. 

\subsection{Evaluation}
To evaluate our model classification performance, we calculated Area Under the Receiver Operating Characteristic Curve (ROC AUC) on the test set with the Sklearn library function. We trained our model for different explanation necessity thresholds, $p_0$, based on the general explanation necessity level for each video. We report the result in Table \ref{tab:model_result}. As shown in the table, the model performance decreases with a lower $p_0$. 

One possible reason is that we are using general explanation scores calculated from different people's ratings. From our user study result (Figure \ref{fig:qualitative-study}), we learned that for dull video scene without any near-crash case, explanation necessity rating tends to have more considerable variance among people, which makes it harder for the model to distinguish scenarios that people do not get an agreement on.

\begin{table}
\caption{Model Performance in terms of test set AUC score. $p_0$ stands for explanation necessity threshold. As shown in the table, the model performs better in high explanation necessity threshold. However, for the low classification threshold, the model performance decreases. }
    \label{tab:model_result}
    \begin{center}
    % \begin{tabular}{ p{1cm} p{3cm} p{3cm}  }
     \begin{tabular}{ @{ }ccc@{ }  }
     \toprule
     \textbf{$p_0$} & \textbf{random guess} & \textbf{our model} \\
     \midrule\midrule
     0.5   & 0.5803    &0.6295 \\ \midrule
     0.6   & 0.5427    &0.6438 \\ \midrule
     0.7   & 0.5359    &0.6794 \\
     \bottomrule
    \end{tabular}
    \end{center}
\end{table}

